Trade-offs in Top-k Classification Accuracies on Losses for Deep Learning

This paper presents an experimental analysis about trade-offs in top-k classification accuracies on losses for deep leaning and proposal of a novel top-k loss. Commonly-used cross entropy (CE) is not guaranteed to optimize top-k prediction without infinite training data and model complexities. The objective is to clarify when CE sacrifices top-k accuracies to optimize top-1 prediction, and to design loss that improve top-k accuracy under such conditions. Our novel loss is basically CE modified by grouping temporal top-k classes as a single class. To obtain a robust decision boundary, we introduce an adaptive transition from normal CE to our loss, and thus call it top-k transition loss. It is demonstrated that CE is not always the best choice to learn top-k prediction in our experiments. First, we explore trade-offs between top-1 and top-k (=2) accuracies on synthetic datasets, and find a failure of CE in optimizing top-k prediction when we have complex data distribution for a given model to represent optimal top-1 prediction. Second, we compare top-k accuracies on CIFAR-100 dataset targeting top-5 prediction in deep learning. While CE performs the best in top-1 accuracy, in top-5 accuracy our loss performs better than CE except using one experimental setup. Moreover, our loss has been found to provide better top-k accuracies compared to CE at k larger than 10. As a result, a ResNet18 model trained with our loss reaches 99 % accuracy with k=25 candidates, which is a smaller candidate number than that of CE by 8.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Top-k_loss_ for ICPR2020 preprint/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Top-k_loss_ for ICPR2020 preprint/topk_paper-cifar100exp_v2.tex <==
We investigated the performance for each loss on more realistic data with deep convolutional neural networks.
\subsection{Settings}\label{sec51}
This experiments was conducted on top-1 and top-5 predictions in 100 classes using the CIFAR-100 dataset \cite{cifar100}, which contains 60,000 RGB images, with 50,000 samples for training and 10,000 for testing. In this experiment, 5,000 training samples were used as the validation set to monitor top-1 or top-5 accuracies across all epochs for early-stopping.

We used a ResNet18 model \cite{resnet} and DenseNet121 model \cite{densenet} to train.
During training, we applied the following data augmentation techniques, random horizontal flips, random crops of size 32 $\times$ 32 on the images zero-padded with 4 pixels on each side, and either Cutout \cite{cutout} (with size 8 $\times$ 8) or Mixup \cite{mixup}. We selected the same learning schedule criteria and hyperparameters of optimization with \cite{cutout}; we used SGD with Nesterov momentum of 0.9, and weight decay of $5\times 10^{-4}$, and  trained for 200 epochs with 128 images per mini batch. The learning rate was initially set to 0.1 and scheduled to decrease by a factor of 5x after each 60th, 120th, and 160th epoch.
%(common for all method, but we see they have all converges before last epoch.)

We evaluated the test accuracies of models both for early-stopping by top-1 validation accuracy and by top-5 validation accuracy. Note that we used two criteria for validation corresponding to the two target metrics of top-1 accuracy and top-5 accuracy respectively. We compared top-1 and top-5 accuracies and other top-k accuracies with different $k$s for better understanding of each loss. Each result is the average over ten trials with different random seeds.

% \subsection{Results}\label{sec52}
\subsection{Results}\label{sec52}

\begin{table*}[!t]
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}
\caption{Test accuracies (\%) on CIFAR-100 dataset. All reported accuracies are averaged over 10 different trials, and values in braces are standard deviations given as uncertainties. Results written in boldface are best ones for each performance metric.}
\label{tab:cifar100_result}
\centering
\begin{tabular}{c|ccccccccccc}
\hline
&\multicolumn{5}{c}{ResNet18}&&\multicolumn{5}{c}{DenseNet121}\\
&\multicolumn{2}{c}{with Cutout}&&\multicolumn{2}{c}{with Mixup}
        &&\multicolumn{2}{c}{with Cutout}&&\multicolumn{2}{c}{with Mixup}\\
Method & Top-1 & Top-5 && Top-1 & Top-5 && Top-1 & Top-5 && Top-1 & Top-5\\
\hline \hline
Cross entropy & \textbf{75.88(0.23)} & 93.11(0.16) && \textbf{76.76(0.23)} & 92.89(0.13)
                    && \textbf{79.05(0.36)} &\textbf{ 94.82(0.15)} && \textbf{79.32(0.25)} & 94.71(0.15) \\
Smooth top-5 SVM \cite{smoothTopK} & 67.31(0.31) & \textbf{93.76(0.12)} && N/A & N/A
                    && 73.55(0.36)& 94.50(0.19) && N/A & N/A \\
Top-5 grouping & 59.99(0.47)&92.64(0.13) && 57.66(0.52) & 92.52(0.21)
                    && 58.69(0.19) & 93.77(0.19) && 56.68(0.94) & 93.58(0.20) \\
Top-5 transition & 69.06(0.30)&93.62(0.18) && 74.26(0.23)&\textbf{94.07(0.14)}
                    && 71.92(0.26) & 94.38(0.24) && 76.28(0.28) & \textbf{95.18(0.06)} \\
\hline
\end{tabular}
\end{table*}

\begin{figure}[!t]
    \centering
    % \includegraphics[trim=60 252 52 300,clip,width=3.5in]{figs_rename/hist_mx_res18_cifar100.pdf}
    \includegraphics[trim=60 252 52 300,clip,width=3.5in]{figs_rename/icpr_cifar100.pdf}
    \caption{Test accuracy of top-k prediction for different $k$. The plot shows the average values over 10 trials of experiment using ResNet18 with Mixup augmentation.}
\label{fig:cifar100_hist}
\end{figure}

The main results are summarized in Table\,\ref{tab:cifar100_result}.
The table shows CE performed the best in top-1 accuracy, as we expected, while its top-5 accuracy was lower than our top-5 transition loss and smooth top-5 SVM loss \cite{smoothTopK} except for the result of DenseNet121 with Cutout. %ここまでが結果
This indicates that trade-offs between top-1 and top-k accuracies occur even on an almost clean dataset, without adding label noises like Berrard \textit{et al.} \cite{smoothTopK}. 
Thus, CE is not always the best choice for training classifiers when we use not only their top-1 but also top-k predictions.

The table also shows that the best top-5 accuracy for each model was obtained by our top-5 transition loss with Mixup, where the improvement from CE was 0.9\,\% for ResNet18 and 0.36\,\% for DenseNet121. 
In the top-5 accuracy with Cutout, smooth top-5 SVM loss \cite{smoothTopK} has shown the slightly higher performance than our top-5 transition loss.
Smooth top-5 SVM loss cannot be directly applied to training on soft label like Mixup, while the top-5 transition loss has better affinity to training techniques. 

The top-5 grouping loss performed worse than CE in both top-1 and top-5 accuracies. 
As we discussed in the synthetic experiments, we consider the reason is that, in CIFAR-100 dataset, inter-class overlap are so small that the top-5 grouping loss cannot select robust decision boundaries.
As a result, the top-5 grouping loss performs worse than CE even in top-5 accuracy. 
In contrast, the top-5 transition loss has realized better top-5 performance than CE and the top-5 grouping loss. 
% Difference between the transition loss and the grouping loss is to initiate the optimization with CE. 
Difference between the transition loss and the top-5 grouping loss is to make transition from CE during optimization.
Therefore, we consider the transition successfully adds a bias to find robust decision boundaries to the top-5 grouping loss. %2文目はtransitionの表現にしたいなあ(swd)

Fig.\,\ref{fig:cifar100_hist} shows top-1 to top-10 accuracies from the results with ResNet18 and Mixup. 
CE loss gives the best top-k accuracy for $k \leq 2$ but defeated by the top-5 transition loss for $k \geq 3$ and also by top-5 grouping for $k \geq 6$.
These turning points consistently appear in the other conditions. 
In the case with DenseNet121 and Cutout CE was the best still in $k=5$, but defeated by the top-5 transition loss for $k \geq 9$ and by the top-5 grouping loss for $k \geq 11$. 
%Top-k transition loss tends to give consistently better performance for $k > 10$ than other losses. %ここが主張
We found the top-5 transition loss gave consistently better performance for $k > 10$ than other losses in all cases.
% The facts indicate that, in the experiments, trade-offs between top-1 and top-k accuracies eventually occur increasing the $k$ for evaluation even when using the grouping loss. %追記 %??? (swd)
% Particularly, our transition loss performs better in top-k accuracy than CE when $k$ is over a certain value. %追記
% Designing a loss for optimizing top-k accuracy on a target $k$ is future work. %追記（いらないかも）
When focusing on fixed target accuracy, the top-5 transition loss can realize 99\,\% with number of prediction candidates $k=25$ saving 8 compared with CE.
This means that using the transition loss reduces the number of candidates for achieving target accuracy, which is preferable characteristic in some practical applications. 
% That characteristic is preferable in some practical applications. 
% practical app = {target k:fixed, target acc:fixed, etc.}

% When focusing on number of candidates to achieve fixed target accuracy,

%To evaluate performance in practical applications, number of prediction candidates necessary for achieving fixed target accuracy is compared. % Settingで書くべき
%(sagi) In oder to evaluate  performance  in  practical  applications,  we compared number of prediction candidates for achieving fixed target accuracy. 
%The evaluation results show that our loss can realize 99\,\% with number of prediction candidates $k=25$ saving 8 compared with CE. %ここまで結果
%Our loss overcomes CE in the practical measure.

%swd なんといっておくのが良いのか難しい。-> Positiveに表現　追加で起こる条件が見つかった、ともいえる
% Although trade-offs between top-1 and top-k accuracy have been observed as in Sec. \ref{sec42}, the condition may not be explained similarly. We observed top-1 training accuracy has reached to almost one, so this setup was not under the condition that a data distribution is complex for a model to fit like Sec. \ref{sec42}.
% The trade-offs have been observed also in deep regime but they were within generalization gap, which is not fully understood with shallow models in our synthetic data experiments.

% To investigate a condition where trade-offs occur in this experiments, top-1 training accuracy was evaluated. %Settingで言うべき？
% As a result, top-1 training accuracies have reached to almost one. % 結果
% The fact indicates that the experimental setups are under the condition that models have sufficient complexity to fit data distribution. %この文から考察
% The condition is different from a condition we found in Sec. \ref{sec42} where trade-offs occur. 
% The fact indicates that trade-offs on experiments on CIFAR-100 comes from a new factor observed in deep regime within generalization gap.

Mechanism behind the trade-offs on CIFAR-100 dataset can not be explained only by the relationship between model complexity and data distribution stated in Sec. \ref{sec44}. 
This is because that top-1 accuracy on the training set reached almost one and thus the models seem to have sufficient complexities to fit top-1 prediction of data distribution.
As discussed in previous paragraphs, the trade-offs also occur in deep learning regime. 
We observed them as the difference in generalization error, not in fitting error caused by insufficiency of model complexity. %できればPOSITIVEに
Further study is needed to understand what makes trade-offs occur in use of deep neural networks.



%sagi One possible reason is generalization gap between training and test dataset. The intra-class overlaps of CIFAR100 are small thus most of data points are classified correctly. This implys that difficult data points near boundaries reduce final accuracy. CE fits models to those difficult training points and thus their boundaries between each class become complex, while our loss designs to obtain smoother boundaries. Therefore we think that our loss can have less generalization gap.

% Mechanism behind the trade-offs on CIFAR-100 dataset can not be explained only the model complexity stated in Sec. \ref{sec42}. This is because that top-1 accuracy reached almost one during training and thus the models seem to have enough complexities to fit the training data distribution. As discussed in previous sections, the  trade-offs also occurs in deep learning regime. However we observed they were within generalization gap. Further study is needed to understand the trade-offs in use of deep models.

% 

% MOVE TO SUPPLEMENT PART ??

% \begin{table*}[!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% \caption{Test accuracies(\%) for losses with margin on CIFAR-100 dataset. All reported accuracies are averaged over 10 different trials, and values in braces are standard deviations given as uncertainties. Results written in boldface are the best ones for each performance metric.}
% \label{tab:cifar100_result_m}
% 	\centering
% 	\begin{tabular}{c|ccccccccc}
% 		\hline
% 		&\multicolumn{4}{c}{Top-1 best validation}&&\multicolumn{4}{c}{Top-5 best validation}\\
% 		Method & Top-1 & Top-3 & Top-5 & Top-7 && Top-1 & Top-3 & Top-5 & Top-7\\
% 		\hline \hline
% 		Cross entropy+ & \textbf{75.70(0.27)}&\textbf{89.21(0.20)}&92.82(0.12)&94.61(0.12)
% 			&&\textbf{75.13(0.48)}&88.97(0.25)&92.81(0.20)&94.59(0.18)\\
% 		Top-5 grouping+ (ours) &63.93(0.39)&87.00(0.31)&92.77(0.23)&95.02(0.18)
% 			&&59.52(0.64)&87.43(0.14)&93.55(0.19)&95.54(0.17) \\
% 		Top-5 transition+ (ours) &70.22(0.32)&\textbf{89.19(0.22)}&\textbf{93.90(0.23)}&\textbf{95.72(0.17)}
% 			&&70.29(0.30)&\textbf{89.16(0.16)}&\textbf{93.86(0.12)}&\textbf{95.72(0.14)} \\
% 		\hline
% 	\end{tabular}
% \end{table*}

% An additional evaluation has been performed for an effect of the margin in multi-class top-k SVM loss.
% Note that outputs from SVM models are unnormalized scores, CE is used in combination with softmax function to train SVMs. %new
% We have introduced the margin term into CE and our losses in the analogy to Berrard's loss \cite{smoothTopK} by regarding our models' logits as scores in SVM.
% The results are seen in Table \ref{tab:cifar100_result_m}.
% It is obvious that the margin improves our top-5 losses further. The best top-5 performance of all evaluations was achieved by our top-5 transition loss with margin.
% Moreover, the transition loss has achieved better top-k accuracy for $k < 5$ without sacrificing top-5 accuracy compared to Smooth top-5 SVM loss \cite{smoothTopK}.
% This is also favorable property in real applications.

% OLD TABLE
% \begin{table*}[!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% \caption{Test accuracies(\%) on CIFAR-100 dataset. All reported accuracies are averaged over 10 different trials, and values in braces are standard deviations given as uncertainties. Results written in boldface are the best ones for each performance metric.}
% \label{tab:cifar100_result}
% \centering
% \begin{tabular}{c|ccccccccc}
% \hline
% &\multicolumn{4}{c}{Top-1 best validation}&&\multicolumn{4}{c}{Top-5 best validation}\\
% Method & Top-1 & Top-3 & Top-5 & Top-7 && Top-1 & Top-3 & Top-5 & Top-7\\
% \hline \hline
% Cross entropy & \textbf{75.88(0.23)} &\textbf{89.41(0.11)}&93.14(0.13)&94.88(0.14)
%                                               &&\textbf{74.52(1.55)}&\textbf{89.11(0.46)}&93.11(0.16)&94.93(0.12) \\
% Smooth top-5 SVM \cite{smoothTopK} &67.31(0.31)&88.46(0.27)&\textbf{93.82(0.08)}&\textbf{95.59(0.10)}
%                                               &&67.12(0.35)&88.43(0.17)&\textbf{93.76(0.12)}&\textbf{95.56(0.06)} \\
% \hline
% Top-5 grouping (ours) & 59.99(0.47)&84.88(0.39)&91.77(0.29)&94.33(0.15)
%                 &&54.57(1.47)&84.94(0.18)&92.64(0.13)&95.00(0.22)\\
% Top-5 transition (ours) & 69.06(0.30)&88.68(0.18)&93.62(0.20)&\textbf{95.55(0.19)}
%                       &&69.07(0.31)&88.65(0.14)&93.62(0.18)&\textbf{95.52(0.11)}\\
% \hline
% \end{tabular}
% \end{table*}

%Smooth top-5 SVM loss \cite{smoothTopK} outperformed CE on the top-5 testing accuracy in this settings even without adding label noises. 
%This loss discards the order in top-k predictions like our top-k loss basically, but it has a margin between correct and incorrect classes originated from multi-class top-k SVM loss \cite{lapin2016}.
%The margin helps to choose robust decision boundary, which seems to benefit also for our top-k losses in test performances.

==> Top-k_loss_ for ICPR2020 preprint/topk_paper-method.tex <==
In this section, we first explain our problem and notations. We then introduce CE and our proposed loss.

\subsection{Problem statements}\label{sec31}
% We consider multi-class classification of $N$ classes with data space $\mathcal{X}$ and label space $\mathcal{Y} = \{1, \cdots, N\}$. Classifiers receive input $x \in \mathcal{X}$ and they return $N$-dimensional vector $\bf{s} \in \mathds{R}^N$ or normalized values $\mathbf{q}$ after softmax operation as their outputs. Top-k prediction for $k=\{1, \cdots, N-1\}$ is a class-label set corresponding to top-k largest components of outputs. We refer to the index sorted in descending order of $\mathbf{q}=\{q_1,q_2,..,q_N\}$ as $[i]\,(i=1, \cdots, N)$, then top-k prediction can be written as
We consider multi-class classification of $N$ classes with data space $\mathcal{X}$ and label space $\mathcal{Y} = \{1, \cdots, N\}$. Classifiers receive input $x \in \mathcal{X}$ and they return $N$-dimensional vector $\bf{s} \in \mathds{R}^N$ or normalized values $\mathbf{q}$ after softmax operation as their outputs. Top-k prediction for $(k=1, \cdots, N-1)$ is a class-label set corresponding to top-k largest components of outputs. We refer to the index sorted in descending order of $\mathbf{q}=(q_1,q_2,..,q_N)$ as $[i]$ for $i=1, \cdots, N$, then top-k prediction can be written as
\begin{align}
\mathcal{C}_k(\bm{q})= \{ y_{[i]} \in \mathcal{Y} | 1 \leq i \leq k \}.
\label{eq-topkpred}
\end{align}
This can cause ambiguity of sorting when an output contains equal components.

Top-k error is now written as an indicator if true label $y$ is not a part of the top-k prediction $\mathcal{C}_k(\mathbf{q})$
\begin{align}
err_k(\bm{q},y) = \mathds{1}[y \notin \mathcal{C}_k(\bm{q})],
\label{eq-topkerr}
\end{align}

where $\mathds{1}$ denotes the indicator function over Boolean statements; 1 if true, 0 if false. Top-k risk is the expectation value of this error. To minimize the risk, we often alter it by a surrogate loss, such as CE or hinge loss, in the optimization.

\subsection{Cross entropy loss}\label{sec32}

CE is the typical surrogate loss of top-1 risk and can be written using the one-hot representation $\textbf{t}$ of $y$ as 
\begin{align}
\mathcal{L}_{CE} = -\log q_y = -\sum_{i=1}^{N}{t_i \log q_i}.
\label{eq-ce1}
\end{align}

The gradients of this function with softmax are dense so that gradient descent in DL works well.

% CEは確率論的に扱えるという話
% Besides, CE loss can be used to minimize distance between probability distributions.%swd よりclear？
% The normalized outputs $q_{i}$s for $i$ are non-negative and sum to 1 so that $q_y$ can model conditional probability of $y$ given $x$. 
% In this sense, cross entropy loss can be seen as $\bm{q}$-dependent part of KL-divergence $D_{KL}$ from $\bm{q}$ to target distribution $\textbf{t}$,
CE can also be used to minimize the distance between probability distributions. The normalized outputs $q_{i}$s for $i$ are non-negative and sum to 1 so that $q_y$ can model the conditional probability of $y$ given $x$. In this sense, CE can be seen as a $\textbf{q}$-dependent part of KL-divergence $D_{KL}$ between $\textbf{q}$ and target distribution $\textbf{t}$,
\begin{align}
\mathcal{L}_{CE}(\bm{q},\bm{t}) = -\sum_{i=1}^{N}{t_i \log q_i} = D_{KL}(\bm{t}||\bm{q})+H(\bm{t}),
\label{eq-ce2}
\end{align}
% where $H(\textbf{t})$ is entropy of $\textbf{t}$. Thus, CE shows how outputs $\textbf{q}$ are different from fixed target $\textbf{t}$ when these values are considered as probability distributions.
where $H(\textbf{t})$ is the entropy of $\textbf{t}$. Thus, CE shows how outputs $\textbf{q}$ differ from $\textbf{t}$ when these values are considered as probability distributions.

CE can be used as the surrogate of top-k risk because it is top-k calibrated for $k>1$ as well as $k=1$ \cite{lapin2016}. This is a preferable property for surrogate loss, which indicates the success in top-k performance of models trained using this loss in DL with large datasets.

However, the calibration does not directly matter for the solutions except minimizers of the loss under ideal resource in data and the complexity of classifiers. Since the optimization process does not always reach such minimizers even in the end of training, it is important to prefer solutions with as small a risk as possible.

% swd　滑らかに入ってこない
There is an extra gap between CE and top-k risk since top-k risk can be zero depending on top-2 to top-k predictions even if top-1 prediction is incorrect. Figure \ref{fig:concept_loss} shows the relation between CE, top-1 risk and top-k risk for a certain data point. CE penalizes top-k correct predictions similarly to incorrect predictions when it is incorrect in top-1 predictions. This leads to a sacrifice in top-k correct prediction on samples difficult to predict correctly in top-1 prediction, instead of achieving top-1 correct prediction on other samples, to minimize the average of losses over all training samples. Therefore, CE is potentially not the best choice to obtain the best top-k accuracy of all possible predictions within practical limitations.



\begin{figure}[!t]
    \centering
    \includegraphics[width=2.5in]{figs_rename/concept_loss.pdf}
    \caption{Schematic view of losses and risks for single data point. Horizontal axis shows output $\textbf{q}$ for true label or most probable class $y$. CE and the proposed top-k grouping loss are plotted in blue and red curves, respectively. Black steps in solid and dotted lines show top-1 risk and top-k risk, respectively. Note that this is1-dimensional slice in $N$-dimensional space of $\textbf{q}$.}
\label{fig:concept_loss}
\end{figure}

\subsection{Top-k transition loss}\label{sec33}
\subsubsection*{\textbf{Top-k class grouping}}\label{sec331}
%\subsection{Top-k grouping loss}\label{sec33}

To obtain a smaller gap onto top-k risk with $k > 1$, we extend CE to derive our top-k loss. Since top-k risk is independent on a ranking in predicted top-k classes, we extend CE to a form independent of the rank. In the extended loss, we do not use original outputs $q_{[i]}$ and target $t_{[i]}$ for the predicted top-k classes $i=1,...,k$ individually. We group these classes as a single class, referred to as top-k union, and use only summations of $q_{[i]}$ for classes in the group instead.


The extended loss, which we call top-k grouping loss $\mathcal{L}_k$, is defined as CE loss calculated for the top-k union and the remaining classes as below,
\begin{align}
\mathcal{L}_{k} = -\left( \sum_{i=1}^{k}{t_{[i]}} \right) \log \left(\sum_{i=1}^{k}{q_{[i]}}\right) - \sum_{i=k+1}^{N}{t_{[i]}\log q_{[i]}}.
\label{eq-topK}
\end{align}

This form ignores the class difference in top-k prediction $\mathcal{C}_k(\textbf{q})$ and permits the confusion in top-k classes. From the viewpoint of probability mentioned in the previous section, the first term is for a probability that an input belongs to one of predicted top-k classes.


This loss has discontinuity at the point where $y$ is getting into the top-k prediction $\mathcal{C}_k(\bf{q})$ because the remaining term changed the input of the logarithm from $q_y$ to the summation of $q_y$ and other $q_{[i]}$s in $\mathcal{C}_k(\bf{q})$. In gradient descent optimization, we can define the gradient on the discontinuous point, for example, as the gradient from the second term.

\subsubsection*{\textbf{Loss transition from CE to top-k grouping loss}}\label{sec332}
%\subsection{Loss Transition between CE loss and Top-k grouping loss}\label{sec34}
The $\mathcal{L}_k$ do not control which classes are contained in top-k predictions, which has an impact on the final test performance. In the early stage of training, the model prediction is uncertain and top-k grouping can be decided at random. There are also possible ways of top-k grouping that can minimize $\mathcal{L}_k$, especially for data distribution in which the classes are well-separated from each other. However, $\mathcal{L}_k$ do not take into account the order of the candidates. Therefore, training only by $\mathcal{L}_k$ will not lead to moderate top-k prediction even if top-k error is minimized for training data. It will be difficult to obtain robust decision boundaries by randomness from possibility, which can be seen as unstable performance in our experiments. %swd exp予言
%It will be difficult to obtain robust decision boundaries by randomness from possibility.

To avoid such risk, we define a loss that uses CE loss at the beginning of training and gradually makes a transition from CE loss to $\mathcal{L}_k$ as follows, 
\begin{align}
\mathcal{L}_{CE,k} = \left(1-\sum_{i=1}^{k}{q_{[i]}}\right)\cdot \mathcal{L}_{CE} + \left(\sum_{i =1}^{k}{q_{[i]}}\right) \cdot \mathcal{ L}_{k}.
\label{eq-transition}
\end{align}


Since $\sum_{i=1}^{k}{q_{[i]}}$ is small for uncertain predictions and becomes closer to 1 as training continues, the transition from CE to our $\mathcal{L}_k$ can be done adaptively with this form with Eq. \ref{eq-transition}. We call this ``top-k transition loss" later in this paper. %swd single to double quote

==> Top-k_loss_ for ICPR2020 preprint/topk_paper-simexp.tex <==

%swd plan
In this section, we explore the possible failure of CE in optimizing top-k prediction by comparing the performance of CE and our top-k losses on simplified settings. Note that we call the top-k grouping loss and the top-k transition loss as top-k losses in this section. To clarify the conditions under where the failure of CE occurs, we investigate the dependency on data distribution and model complexity.

First, we focused on the data distribution dependency with a fixed model. In Experiment 1, we used the simple data distribution, where each class comes from a single normal distribution, located on a circle, with different inter-class overlap. We extended this to a more complex distribution in Experiment 2, by adding a minor mode to each class distribution at a different distance from the major mode. 

Next we examined the dependency on model complexity in Experiment 3 using the data distribution that was found to cause sub-optimal top-k performance of CE in the preceding experiments.
Detailed setups and discussions for each experiment are described in the following subsections.

\subsection{Experiment 1: On class confusion}\label{sec41}
In this experiment, we examined the performance of CE and the top-k losses on different strengths of inter-class confusion that increase the top-1 risk of the best possible prediction, which can be trained with a model having infinite complexity. We set $k=2$ in six classes.

\subsubsection*{\textbf{Settings}}

We used the synthetic data distribution that consists of normal distributions with standard deviation $\sigma$ on the circle of radius 1, each mode belongs to each class respectively. Let $\theta$ be the parameter that indicates the position on the circle as the angle from one of the positive axes in data space. We have six classes and their centers are placed at equal spaces 60$\,^{\circ}$ in $\theta$. Parameter $\sigma$, which controls confusion strength, is changed to 10$\,^{\circ}$, 15$\,^{\circ}$, 20$\,^{\circ}$, 25$\,^{\circ}$, and 30$\,^{\circ}$. The number of confusing classes at each data point varies as $\sigma$ changes. We sampled 300 data points per class from the distribution both for training and evaluation data. 

Figure \ref{fig:sim_dataset_a} shows an example of the data distribution when $\sigma$ was set to 20$\,^{\circ}$. In this case, there are about two confusing classes at any data point since the tail at 99.7 \% of each normal distribution reaches the center of the neighbor class distribution. Note that inter-class confusion decreases the best possible top-1 accuracy for each data point up to the ratio of class.

For a classifier, a neural network composed of a two-dimensional input layer, a fully connected layer to six dimensions without bias terms, and an activation layer with softmax function was used. The network was trained for 1,000 epochs.

We report on the test accuracies averaged over ten runs with different random seeds in sampling the datasets and training the networks. The top-1 and top-2 performances for CE, the top-2 grouping loss, and the top-2 transition loss were compared at each $\sigma$. 

% (Results and discussion)

\begin{figure*}[!t]
    \centering
    \subfloat[Sampled dataset]{\includegraphics[width=2.3in]{figs_rename/exp0_datahist.pdf}%s1a
    \label{fig:sim_dataset_a}}
    \hfil
    \subfloat[Top-1 accuracy]{\includegraphics[width=2.3in]{figs_rename/exp0_top-1acc.pdf}%s2a
    \label{fig:sim1a}}
    \hfil
    \subfloat[Top-2 accuracy]{\includegraphics[width=2.3in]{figs_rename/exp0_top-2acc.pdf}%s2b
    \label{fig:sim1b}}
    \caption{Results from Experiment 1 for different widths of single class mode $\sigma$. (a) Example of sampled data $\sigma=20\,^{\circ}$. (b) Top-1 and (c) top-2 accuracies by each loss.}
\label{fig:sim1}
\end{figure*}

\subsubsection*{\textbf{Results}}

Figure \ref{fig:sim1} shows the top-1 and top-2 accuracies of the network trained by each loss for different $\sigma$. The error-bar shows maximum and minimum accuracies in the trials. In top-2 accuracy as well as in top-1 accuracy, CE obtained almost the best  of all losses in this settings. We can see in top-1 and top-2 accuracies a tendency that CE performed better than our losses, especially for $\sigma<20\,^{\circ}$, where inter-class overlaps are small. For such a non-overlapping region, the top-2 losses cannot uniquely determine top-2 class combination to predict. This leads to not only low top-1 accuracy but also no robust boundary of the top-2 combination in contrast to CE. For this reason, the top-2 accuracy of our losses degrades on average when there is a discrepancy between training and test data. This can be seen as large error-bar on $\sigma=15\,^{\circ}$ in Fig. \ref{fig:sim1b} due to large degradation in a few trials.

The performance of the top-2 losses asymptotically approached CE for $\sigma\geq 20\,^{\circ}$, where more than two classes significantly overlap. With large overlaps, the top-2 losses can find which combination of top-2 classes to predict over almost all data points and decision boundaries similar to that of CE. As a result, accuracies of the network trained the top-2 losses approached CE for large $\sigma$.

% コメント by e-kaneko
% 今回の話の場合、"decision boundary"が2種類あり得る。
% 一つは通常通り上位１位クラスの境界。もう一つは上位2位クラスの組み合わせの境界。
% なので、ここで初出のdecision boundaryがどちらを意味するかはっきりわかるように書きたい。

\subsection{Experiment 2: On multi-modality of distribution}\label{sec42}
The failure of CE in top-2 performance was not found in Experiment 1 where confusion strength was controlled with the optimal prediction boundary fixed. In this experiment, we considered a more complex data distribution by adding a minor mode to each class distribution. We set $k=2$ in six classes, as in Experiment 1.
% 具体例書きたい

\subsubsection*{\textbf{Settings}}
We used the same data distribution as in Experiment 1 with $\sigma=10\,^{\circ}$ as major modes. Unlike experiment 1, each class had an additional minor mode of normal distribution2 times less frequent as the major mode with the same width. Each minor mode is located with shift in $d$ from the major mode of the same class, and $d$ is changed to 30$\,^{\circ}$, 45$\,^{\circ}$, 60$\,^{\circ}$, 75$\,^{\circ}$ and 90$\,^{\circ}$. Dataset sampling, training, and evaluation were carried out in the same manner as in Experiment 1. The same model architecture as also used. The top-1 and top-2 performances for CE, the top-2 grouping loss, and the top-2 transition loss were compared at each $\sigma$. 

Figure \ref{fig:sim_dataset_b} shows an example of the data distribution for this experiment for $d=90\,^{\circ}$. Under this condition, each minor mode was located between the major modes of the nearest and next nearest neighbor classes. The minor modes make additional split regions of optimal prediction.

%書き方がわからない！！optimal predictionの存在への布石を置きたい

% (Results and discussions)

\begin{figure*}[!t]
    \centering
    \subfloat[Sampled dataset]{\includegraphics[width=2.3in]{figs_rename/exp1_datahist.pdf}%s1b
    \label{fig:sim_dataset_b}}
    \hfil
    \subfloat[Top-1 accuracy]{\includegraphics[width=2.3in]{figs_rename/exp1_top-1acc.pdf}%s2a
    \label{fig:sim2a}}
    \hfil
    \subfloat[Top-2 accuracy]{\includegraphics[width=2.3in]{figs_rename/exp1_top-2acc.pdf}%s2b
    \label{fig:sim2b}}
    \caption{Results from Experiment 2 for different inter-mode distance $d$. (a) Example of sampled data $d=90\,^{\circ}$. (b)Top-1 and (c) top-2 accuracies by each loss.}
\label{fig:sim2}
\end{figure*}


\subsubsection*{\textbf{Results}}

Figure \ref{fig:sim2} shows the top-1 and top-2 accuracies of the network trained by each loss for different $d$. We can see the trade-off between top-1 and top-2 accuracies for $d>60\,^{\circ}$.
From region $d<45\,^{\circ}$, CE is superior to the top-2 losses both in top-1 and top-2 accuracies. The distribution of each class only becomes asymmetric due to the minor mode in this region, which can be understood in the same manner as in Experiment 1 with small $\sigma$.
On the other hand, we can see that CE is inferior to the top-2 losses in top-2 accuracy for $d\geq 60\,^{\circ}$, which is the case in which CE failed to obtain the best possible top-2 accuracy.

% コメント by e-kaneko
% asymmetricになった「だけ」のexp1であるのは正しいけど、
% この「only=だけ」の背後に、「exp1と同様、optimalなsolutionがsplitされていないこと」が隠れている。
% この条件がより大事なポイントなので、追記したい。

%While top-1ではずっとbestってどっかに追加したい by swd

\subsection{Experiment 3: On model complexity}\label{sec43}
In this experiment, we explored the dependency on model complexities that were fixed in the two experiments above. 

\subsubsection*{\textbf{Settings}}
We used the same data distribution as in Experiment 2 for $d=90\,^{\circ}$, where CE failed to fit the optimal top-2 prediction. Dataset sampling, training, and evaluation were carried out in the same manner as in Experiments 1 and 2.

The model architecture was different from that used in the above experiments, a hidden layer followed by ReLU activation were inserted after the input layer. To control model complexity, we changed the number of nodes $m$ for the hidden layer, i.e., 2, 4, 8, 16, and 32. The average top-1 and top-2 accuracies for CE, the top-2 grouping loss, and the top-2 transition loss were compared for each $m$.

%(Results and discussion)

\begin{figure*}[!t]
    \centering
    \subfloat[Top-1 accuracy]{\includegraphics[width=2.5in]{figs_rename/exp3_top-1acc.pdf}%
    \label{fig:sim3a}}
    \hfil
    \subfloat[Top-2 accuracy]{\includegraphics[width=2.5in]{figs_rename/exp3_top-2acc.pdf}%
    \label{fig:sim3b}}
    \caption{Results from Experiment 3 for different number of nodes in hidden layer $m$. (a)Top-1 and (b) top-2 accuracies for each loss.}
\label{fig:sim3}
\end{figure*}

\subsubsection*{\textbf{Results}}

Figure \ref{fig:sim3} shows the top-1 and top-2 accuracies of the network trained by each loss for different $m$. The top-2 performance by CE was not the best of all losses for low complexity $m\leq4$, the same as in Experiment 2. For higher complexity $m\geq 8$, CE achieved the best performance both in top-1 and top-2 accuracies.

% Visualization part here in the past

\subsection{Visualization of resulting predictions}\label{sec44b}

\begin{figure*}[!t]
    \centering
    \subfloat[Experiment 2 for $d=90\,^{\circ}$ ]{\includegraphics[width=3.0in]{figs_rename/exp1_pred.pdf}%s4
    \label{fig:sim_analysis_a}}
    \hfil
    \subfloat[Experiment 3 for $m=8$]{\includegraphics[width=3.0in]{figs_rename/exp3_pred.pdf}%s6
    \label{fig:sim_analysis_b}}
    \caption{Visualization of data distribution and resulting predictions by each loss (a) in Experiment 2 for $d=90\,^{\circ}$ and (b) in Experiment 3 for $m=8$. Predictions for class 2 are shown with bars at top of each figure.}
\label{fig:sim_analysis}
\end{figure*}

To take a closer look at the failure of CE in top-2 accuracy, Figures \ref{fig:sim_analysis_a} and \ref{fig:sim_analysis_b} visualize expected data distributions and the resulting predictions for a case of $d = 90 \,^{\circ}$ in Experiments 2 and 3, respectively. Lines at the bottom of each figure are the data distributions. Focusing on the class indicated as the green line, the shaded area shows where the class is the most frequent. Thick and thin horizontal bars above the distributions show top-1 and top-2 predictions of the target class for each loss, respectively.

Figure \ref{fig:sim_analysis_a} is for a network without any mid-layers. The top-2 grouping loss and the top-2 transition loss cover all the green area, while CE does not. In contrast, CE has a better top-1 prediction than our loss in a major mode. These results indicate that CE does not optimize top-2 prediction when data has a more complex distribution than the model complexity. Moreover, our losses can perform better in top-2 prediction sacrificing top-1 prediction.

Figure \ref{fig:sim_analysis_b} is same as Fig. \ref{fig:sim_analysis_a} except for the case containing a mid-layer with nodes of $m=8$ in Experiment 3. In contrast to Fig. \ref{fig:sim_analysis_a}, there are two split areas of top-1 prediction for all losses corresponding to a true data distribution. All losses cover the most frequent region for the target class, that is, they obtained almost optimal top-2 predictions. Moreover, top-1 prediction of CE represents optimal top-1 prediction well. This shows that the network with nodes of $m \ge 8$ has sufficient complexity to fit optimal top-1 prediction for this data distribution, unlike the network in Experiment 2. This suggests that CE can obtain the best possible top-2 predictions when we use models complex enough to fit optimal top-1 prediction.

%\subsection{Brief summary of the synthetic data experiments}\label{sec44}
\subsection{Brief summary}\label{sec44}
We summarize our findings from the experiments on synthetic data.

According to the results from Experiments 1 and 2, CE can suffer from the trade-off between top-1 and top-k performances when the data distribution has complex structures. The inter-class confusion is not an essential component that caused top-k failure of CE in Experiment 1 while the optimal risk increased. We found that CE does not perform well in top-k accuracy when the distribution of a certain class has multiple modes that leads to a complex decision boundary to achieve optimal top-1 prediction, which can be observed in practical data.

%From Experiment 3, we saw that the critical complexity of data distribution depends on the complexity of the model to train. If the model can fit the optimal top-1 decision boundary for a given data distribution, CE loss may give optimal prediction in not only top-1 but also top-k accuracy.
% In Experiment 3, we saw that such trade-off disappeared when using more complex models that can fit the optimal top-1 decision boundary for a given data distribution. It is suggested that CE loss leads to almost optimal top-k prediction as well as top-1 prediction with enough model complexity. %swd
Experiment 3 showed that such trade-off does not occur when using more complex models that can fit the optimal top-1 decision boundary for a given data distribution. It is suggested that CE leads to almost optimal top-k prediction as well as top-1 prediction with enough model complexity. %sagi
% disappearedという言葉に若干違和感。それとmore complex modelとしているが、比較級を使う必要もない気がする。
% コメントアウトしてるのは変更案

% ロジックやワードに飛躍を感じる
% 前後の段落との流れがスムーズになるようにしたい
% 段落ごとのトピック文が飛躍なくつながるようにして、その内容に合うような文章にしたい
% 例えばこんな感じのトピックセンテンス
% 前段落：「実験1,2から、データ構造が複雑なときにCEがtop-k予測で最適ではないことがわかった」
% この段落：「実験3から、モデルの表現力が足りないときにも、CEはtop-k予測で最適ではないことがわかった」
% 後段落：「結論として、データが複雑で、モデルがそれを表現する複雑さを持たないとき、CEはtop-k予測で最適ではないことがわかった」

%After all, CE loss is not an optimal loss for learning top-k prediction when we have complex data distribution for a model to fit. Our losses can achieve better top-k accuracy under such conditions.
% After all, CE loss is not always an optimal choice to learn top-k prediction and it happens for example when a model is too poor to fit the optimal top-1 prediction of a data distribution. Our losses can achieve better top-k accuracy under such conditions. %swd
After all, CE loss is not always an optimal choice to learn top-k prediction and it happens for example when a model does not have sufficient complexity to fit top-1 prediction of a data distribution. Our losses can achieve better top-k accuracy under such conditions. %kaneko


%swd ロジックは変わっていないように私は見えてしまうので、ワードで見るとthe critical complexity of data distributionが唐突感あるでしょうかね。下記だとマシですか？
%（頭サチり人間なので、どこが飛躍と感じるかを特に書いておいてほしいです）

%1 According to the results from Experiments 1 and 2, CE can suffer from the trade-off between top-1 and top-k performances when the data distribution has complex structures.
% ここは存在を示すところからなのでこの順で述べたい

%2 From Experiment 3, we saw that such trade-off disappeared when using more complex models.

%3 After all, CE loss is not an optimal loss for learning top-k prediction when we have complex data distribution for a model to fit.
% 存在を示すところ＋実験から推測される発生条件を述べたい

% ekaneko 
% ワードがtrade-offになっただけでだいぶ飛躍感は消えました。
% ですが、まだ2と3の間に飛躍を感じます。
% 1,2,3を日本語でざっくり訳すと、こんな感じ
% 1:「実験１，２によれば、CEは、データ構造が複雑なときにトレードオフを被る」
% 2:「実験3によれば、そのトレードオフは、複雑なモデルを使うと消える」
% 3:「つまり、CEは、モデルがフィットできないほど複雑なデータのときに最適なロスではない」
% 1,2がこの内容であれば、3で言えるのは以下くらい。
% 「CEのトレードオフは、データが複雑かつモデルが簡単なときにおこる」
% でも3ではもうちょっと言いたい。
% 特に「モデルがフィットできないほど複雑なデータのときに」というニュアンスを入れたい
% この表現は実験3の考察で触れているので2で言い切っちゃってはどうか。
% 例えば
% 2: 「実験3の考察によれば、そのトレードオフは、モデルがフィットできないほど複雑なデータのときに生じる」
% とすれば、
% 3はこれくらい言える
% 「すなわち、モデルがデータの複雑さを表現しきれないときには、CEはtop-kよそくで最適ではない」
% この方向で進めるのはどうでしょうか

% swd どこまでをトピックセンテンスに突っ込むかですね。2のところは確かに後に書いてしまっているので、
% 2: 「実験3(の考察)によれば、そのトレードオフは、モデルがフィットできないほど複雑なデータのときに生じる」（モデルが十分複雑、考察によると特にtop1をfitできるくらい複雑な時、）
% とするのは賛成です。
% ただ、ここの接続性だけを見て「トレードオフの存在を示すところ」が抜けた言い方にならないようにはしたいですね

% ekaneko
% 「トレードオフの存在を示す」ということを明示的に結論に入れたい件、了解しました。
% であれば、3はこんな感じ
% 3:「すなわち、CEによる学習では〇〇と〇〇のトレードオフが生じ得るし、それはモデルがデータの複雑さを表現しきれないときに起こる」

